AcTune: Uncertainty-aware Active Self-Training for Semi-Supervised Active Learning with Pretrained Language Models

While pre-trained language model (PLM) fine-tuning has achieved strong performance in many NLP tasks, the fine-tuning stage can be still demanding in labeled data. Recent works have resorted to active fine-tuning to improve the label efficiency of PLM fine-tuning, but none of them investigate the potential of unlabeled data. We propose {\ours}, a new framework that leverages unlabeled data to improve the label efficiency of active PLM fine-tuning. AcTune switches between data annotation and model self-training based on uncertainty: it selects high-uncertainty unlabeled samples for active annotation and low-uncertainty ones for model self-training. Under this framework, we design (1) a region-aware sampling strategy that reduces redundancy when actively querying for annotations and (2) a momentum-based memory bank that dynamically aggregates the model's pseudo labels to suppress label noise in self-training. Experiments on 6 text classification datasets show that AcTune outperforms the strongest active learning and self-training baselines and improves the label efficiency of PLM fine-tuning by 56.2\% on average. Our implementation will be available at \url{https://github.com/yueyu1030/actune}.

==> 01intro.tex <==
\section{Introduction}
While pre-trained language models have achieved enormous success in natural language processing (NLP), they are usually label-hungry, and often require thousands, or even millions of labeled instances to achieve satisfactory performance. 
In practice, however, obtaining such an amount of labeled data can be prohibitively expensive. 
This has become the biggest hurdle that prevents deep learning models from being deployed for many NLP tasks in various domains.

% introducing AL and Self Training
To relieve the label scarcity bottleneck, active learning (AL) is a paradigm for label-efficient learning  with massive unlabeled data. 
Specifically, active learning approaches train a model on a small set of labeled data and select the most representative samples in unlabeled data to label in an iterative manner~\cite{settles2011theories}. 
In this way, they are able to achieve comparable performance to fully-supervised methods while requiring few annotated samples.
Active learning has been applied to various NLP tasks including text classification~\cite{ein-etal-2020-active,yuan-etal-2020-cold}, sequence labeling~\cite{shen-etal-2017-deep,radmard-etal-2021-subsequence,shelmano2021active}, question answering~\cite{lin2017active,karamcheti2021mind} and machine translation~\cite{zhao2020active} with promising performance.

So far, several studies aim to improve the AL method from different perspectives.
\emph{Uncertainty-based} methods \citep{holub2008entropy,gal2017deep,balm,margatina2021active,ru2020active,shelmano2021active} measure the uncertainty for each sample based on model's predictions, and select the most uncertain examples for annotation. 
In contrast, \emph{diversity-based} methods~\cite{coreset,yuan-etal-2020-cold} select the most representative samples which best approximate the full dataset. 
There are also some \emph{hybrid} methods that combine diversity and uncertainty sampling~\cite{badge,kirsch2019batchbald}. 
Despite they achieving superior performance over random sampling baselines, these approaches still have several drawbacks: 
(1) Although they query the labels for only a small fraction (e.g. 10\%) of the data, however, for large-scale datasets, annotating such a number of examples can still be prohibitively expensive. 
Take AGNews~\cite{zhang2015character} as an example, querying 10\% of the data requires more than 10,000 annotated examples, which is still costly; 
(2) They neglect unlabeled data during training the downstream model, while unlabeled data is potentially useful to further promote the model performance when labeled data is scarce~\cite{du-etal-2021-self,vu2021strata}; 
(3) They are still sensitive to outliers~\cite{karamcheti2021mind}. Outliers naturally have large model uncertainty, but querying their labels brings limited gain in overall performance improvement. To sum up, it is still challenging to design effective active learning methods under the low-data regime. 

% challenge: (1) Unlabel, (2) mid-data region (3) outlier

\cite{karamcheti2021mind}
\cite{siddhant2018deep}
\cite{zhang2021cartography}
\cite{song2019combining}
\cite{mittal2019parting}

There are several lines of research targeting improving the label efficiency: One line of the research uses \emph{active learning} technique to identify the most relevant examples in unlabeled data and query their labels from the oracle~\cite{ein-etal-2020-active,yuan-etal-2020-cold,balm,margatina2021active}. 
Meanwhile, another line of methods focuses on \emph{few-shot learning}, which aims to improve the model's generalization ability with limited labeled data and a large number of unlabeled data~\cite{mukherjee2020uncertainty,wang2021meta,xie2020unsupervised,vu2021strata}.  
Although all of these methods attempt to better leverage the power of unlabeled data to iteratively improve the prediction performance, they utilize the unlabeled data in a totally different way: the former methods acquires labels for \emph{most  uncertain} or \emph{diverse} samples, 
while the latter bootstraps on unlabeled examples with \emph{most confident} model predictions. 
Consequently, a natural question arises: \emph{Can we combine the advantage of active learning and few-shot learning together to tackle the label scarcity bottleneck?}

% emphasize the limitation of existing methods
So far, there are several works aiming to combine these two techniques together~\cite{tomanek2009semi,rottmann2018deep,simeoni2021rethinking,gao2020consistency,mittal2019parting}. 

Progressive Refine
\cite{qin2021knowledge,gu-etal-2021-transformer,gong2019efficient}
% Our method

\cite{gao2020consistency}
\cite{tomanek2009semi}

% Exp

